COMET: Generating Commit Messages using Delta Graph Context Representation

Commit messages explain code changes in a commit and facilitate collaboration among developers. Several commit message generation approaches have been proposed; however, they exhibit limited success in capturing the context of code changes. We propose Comet (Context-Aware Commit Message Generation), a novel approach that captures context of code changes using a graph-based representation and leverages a transformer-based model to generate high-quality commit messages. Our proposed method utilizes delta graph that we developed to effectively represent code differences. We also introduce a customizable quality assurance module to identify optimal messages, mitigating subjectivity in commit messages. Experiments show that Comet outperforms state-of-the-art techniques in terms of bleu-norm and meteor metrics while being comparable in terms of rogue-l. Additionally, we compare the proposed approach with the popular gpt-3.5-turbo model, along with gpt-4-turbo; the most capable GPT model, over zero-shot, one-shot, and multi-shot settings. We found Comet outperforming the GPT models, on five and four metrics respectively and provide competitive results with the two other metrics. The study has implications for researchers, tool developers, and software developers. Software developers may utilize Comet to generate context-aware commit messages. Researchers and tool developers can apply the proposed delta graph technique in similar contexts, like code review summarization.

==> 02_background.tex <==
\section{Background}
% This figure belongs to Methods section; put it here so that we see it from the right page.


In this section, we briefly discuss relevant concepts and techniques used in the presented work.

\subsection{Version Control Systems and Commit Messages}
A Version Control System (\textsc{vcs})~\parencite{Spinellis2005} 
is responsible for recording and managing the changes that occur in digital artifacts such as computer programs and documents.
% and for maintaining a record of different versions of the same documents. 
Prominent examples of \textsc{vcs}s are Git, \textsc{tfs}, and \textsc{svn}.
Typically, a \textsc{vcs} creates a \textit{repository}
that represents a database to store metadata of the changes in each version.
A developer creates a \textit{commit} to record the changes in the repository; 
a \textit{commit message} is the description and rationale of the recorded changes, \ie{} a commit, in natural language text.

% push their changes onto the repository maintained in the VCS tool accompanied by a commit message. A commit message is a concise yet informative summary of the changes made to the source code of a project, written in natural language.

\begin{comment}
\todo{reduce this section, we dont contribute anything regarding LLM}
\subsection{Large Language Models}
Large Language Models (\textsc{llm}s) are advanced deep learning models that have been trained on large amounts of text data, 
allowing them to learn complex patterns and relationships in a language. 
They have been used in a variety of language-specific tasks, such as 
question-answering~\cite{pearce2021} and
text summarization~\cite{liu2019, muennighoff2022}. 
Popular examples of \textsc{llm}s include \textsc{gpt}-3~\cite{brown2020}, 
BERT~\cite{devlin2019}, 
T5~\cite{raffel2020}, and
LLaMA~\cite{touvron2023}. 
% \todo{Add a couple of sentences for code specific LLMs}
%Users can take advantage of these models by fine-tuning them on their own datasets for specific downstream tasks saving both time and computational resources compared to training models from scratch. 
Fine-tuning a language model allows users to leverage the pre-trained models' existing knowledge and adapt it to their specific use cases, making it a powerful tool for various tasks. \textsc{llm}s have also proved to be effective in software engineering tasks such as code summarization \cite{ahmad2020transformer}, code generation ~\cite{Svyatkovskiy2020}, and defect prediction ~\cite{Li2017}. For instance, CodeBERT~\cite{feng2020} is a variant of \textsc{bert}~\cite{devlin2019} that has been fine-tuned on a large code corpus, making it specifically suitable for code-related tasks. On the other hand, GraphCodeBERT~\cite{guo2021} is a pre-trained model that considers the inherent structure of code by encoding the data flow relation between variables, enhancing the code understanding process beyond token-level syntax analysis~\cite{guo2021}.
% TS: Nice paragraph (above)

\end{comment}
\subsection{Code Property Graph}
Code Property Graph (\cpg{})~\parencite{yamaguchi2014} merges classic program analysis concepts Abstract Syntax Trees (\abst{}s), 
Control Flow Graphs (\cfg{}s), 
and Program Dependence Graphs (\pdg{}) into a single, 
graph-based representation of code along with its context. 
\cpg{}s capture essential code properties such as syntax, semantics, data flow, and control flow making them an effective tool for analyzing and understanding code.

\begin{comment}
\subsection{Graph Neural Networks}
Graph Neural Networks (\gnn{}s)~\cite{Scarselli2009} operate on graph-structured data and capture complex relationships between entities effectively.
% \gnn{}s excel in code-specific tasks \cite{Siow2022}
\gnn{}s learn node and edge representations by aggregating information from their local neighborhoods, 
enabling them to model complex relationships among nodes in the graph. 
\gnn{}s have demonstrated promising results in various graph-related tasks, 
including node classification~\cite{bhagat2011}, 
link prediction~\cite{liben2003}, and graph classification~\cite{errica2019}.

\subsection{Convolutional Neural Networks}
Convolutional Neural Networks (\cnn{}s) have been widely used for image-related tasks such as image classification~\cite{lu2007}, object detection~\cite{zou2023}, and image segmentation~\cite{minaee2021}.
\cnn{}s can learn spatial hierarchies of features by convolving the input sample with a set of filters.
Recently, \cnn{}s have also been used for various code-specific tasks such as defect prediction~\cite{Li2017}.
\end{comment}

% \todo{do we want to somehow combine transformer section with LLM section; there is good portion of overlap}
\subsection{Transformers} 
% \todo{Remove this as transformer is well known?}
Transformers are a type of neural network architecture that has become increasingly popular in natural language processing tasks due to their ability to process input sequences in parallel and handle long-range dependencies more effectively than traditional recurrent neural networks~\parencite{Vaswani2017}. 
The transformer architecture comprises an encoder and a decoder, each consisting of multiple layers of self-attention and feedforward neural networks. 
% \todo{I feel this reduction makes sense: Please check commented text}
% \doubt{@Tushar}
%The encoder processes the input sequence and generates a fixed-length representation called the context vector. The decoder then takes the context vector and generates the output sequence one token at a time.
%In addition to natural language processing, transformers have also been used in various software engineering tasks, 
%such as code summarization~\cite{ahmad2020transformer}, 
%code generation~\cite{Svyatkovskiy2020}, and defect prediction~\cite{Fu2022}. 
The attention mechanism, which is a key component of transformers, 
allows the model to selectively focus on parts of the input sequence that are most relevant to the current task. 
This makes transformers effective in processing both sequential and non-sequential data, such as graphs, by allowing them to selectively attend to important nodes or edges a graph structure.

% \subsection{Motivation}
% \todo{move this to introduction}
% Even though a lot of work has already been done in the direction of commit message generation, there are still issues that need to be addressed. Some of the issues that acted as a motivation for us to pursue this work are:
% \begin{itemize}
% \item Low-Quality Training Dataset: Data used to train the commit generation models usually consists significant proportion of improper messages that eventually reflects in the model’s performance.
% \item Treating code as a sequence of tokens: Current solution
